Understanding the Distributions of Aggregation Layers in Deep Neural Networks

The process of aggregation is ubiquitous in almost all deep nets models. It functions as an important mechanism for consolidating deep features into a more compact representation, whilst increasing robustness to overfitting and providing spatial invariance in deep nets. In particular, the proximity of global aggregation layers to the output layers of DNNs mean that aggregated features have a direct influence on the performance of a deep net. A better understanding of this relationship can be obtained using information theoretic methods. However, this requires the knowledge of the distributions of the activations of aggregation layers. To achieve this, we propose a novel mathematical formulation for analytically modelling the probability distributions of output values of layers involved with deep feature aggregation. An important outcome is our ability to analytically predict the KL-divergence of output nodes in a DNN. We also experimentally verify our theoretical predictions against empirical observations across a range of different classification tasks and datasets.

==> backup.tex <==
\begin{figure}
    \centering
    \begin{tabular}{ccc}
    Average Pool & Exp. Pool & KL-Div.\\
    \includegraphics[width=0.3\linewidth]{imgs/cifar_out_cls9.pdf} & \includegraphics[width=0.3\linewidth]{imgs/cifar_exp_out_cls9.pdf} & 
    \includegraphics[width=0.3\linewidth]{imgs/cifar_kl.pdf}
    \end{tabular}
    CIFAR Dataset \\
    \begin{tabular}{ccc}
    %Average Pool & Exp. Pool & KL-Div.\\
    \includegraphics[width=0.3\linewidth]{imgs/flower_rose_avp.pdf} & \includegraphics[width=0.3\linewidth]{imgs/flower_rose_exp.pdf} & 
    \includegraphics[width=0.3\linewidth]{imgs/flowers_kl.pdf}
    \end{tabular} \\
    Flowers Dataset\\
    \begin{tabular}{ccc}
    %Average Pool & Exp. Pool & KL-Div.\\
    \includegraphics[width=0.3\linewidth]{imgs/eyepacs_avpool.pdf} & \includegraphics[width=0.3\linewidth]{imgs/eyepacs_exppool.pdf}  &
    \includegraphics[width=0.3\linewidth]{imgs/eyepacs_kl.pdf}
    \end{tabular} \\
    EyePACs Dataset
    \caption{Examples of predicted output node distributions (red and black curves) and observed underlying histograms. Black represents images with negative labels, whilst red represents images with positive labels. The rightmost plot shows the scatter plots of predicted (x-axis) against observed (y-axis) KL-divergence of the DNN output node.The green diagonal line on the right plot indicates when the predicted and observed KL divergence are equal. Blue circles indicate exponential activation, and black crosses indicate average pooling.}
    
    \label{fig:kl_plot}
\end{figure}






% APPENDIX DEACT MEAN VARIANCE OLD
\section{Deactivation Distribution Mean and Variance}
The mean of $w(x)$ (Thm. \ref{thm:deact_pdf}), denoted as $\mu_w$ is found as follows:
\begin{eqnarray*}
\mu_w & = & \frac{1}{\gamma\Gamma(a)s^a}\int^\infty_0
x^{\frac{a-\gamma}{\gamma}}\exp\left(-\frac{x^{1/\gamma}}{s}\right) x\; dx\\
& = & \frac{1}{\gamma\Gamma(a)s^a}\int^\infty_0
x^{\frac{a}{\gamma}}\exp\left(-\frac{x^{1/\gamma}}{s}\right) dx
\end{eqnarray*}
Performing change of variables with $y = x^{1/\gamma}/s$, so $dy/dx = (1/(\gamma s))x^{1/\gamma - 1}$ and $w(0) = 0$, resulting in the integral:
\begin{eqnarray*}
\mu_w & = & \frac{1}{\gamma\Gamma(a)s^a}\int^\infty_0 \exp(-y) x^{a/\gamma} s x^{1 - 1/\gamma} dy \\
& = & \frac{1}{\gamma\Gamma(a)s^a}\int^\infty_0 \exp( -y) x^{1 + (a-1)/\gamma} dy \\
& = & \frac{1}{\gamma\Gamma(a)s^a}\int^\infty_0 \exp( -y) y^{\gamma + a - 1} dy \\
& = & \frac{s^\gamma\Gamma(\gamma + a)}{\Gamma(a)}
\end{eqnarray*}

To find the variance, we first find the second moment (denoting the random variable as $X_w$):
\begin{eqnarray*}
\mathbb{E}[X_w^2] & = & \frac{1}{\gamma\Gamma(a)s^a}\int^\infty_0
x^{\frac{a-\gamma}{\gamma}}\exp\left(-\frac{x^{1/\gamma}}{s}\right) x^2\; dx
\end{eqnarray*}
Similar to the mean, changing the variable with $w = x^{1/\gamma}/s$ results in the integral becoming:
\begin{eqnarray*}
\mathbb{E}[X_w^2] & = & \frac{s^{2\gamma}}{\Gamma(a)} \int^\infty_0 y^{a -1 + 2\gamma} e^{-y} dy \\
& = & \frac{s^{2\gamma}\Gamma(a + 2\gamma)}{\Gamma(a)}
\end{eqnarray*}
where the last line again used Eq. \ref{eq:int_lemma} from Lemma \ref{lem:int_lemma}.

 Finally, substituting the above second moment and mean into Eq. \ref{eq:gen_var} results in the required variance, denoted as $\sigma^2_e$:
\begin{eqnarray*}
\sigma^2_e & = & \frac{s^{2\gamma}\Gamma(a + 2\gamma)}{\Gamma(a)} - \left( \frac{s^\gamma\Gamma(\gamma + a)}{\Gamma(a)} \right)^2 \\
& = & \frac{s^{2\gamma}\Gamma(a + 2\gamma)}{\Gamma(a)} - \frac{s^{2\gamma}\Gamma( a + \gamma)^2}{\Gamma(a)^2} \\
& = & \frac{s^{2\gamma}}{\Gamma(a)}\left( \Gamma(a + 2\gamma) - \frac{\Gamma(a+\gamma)^2}{\Gamma(a)}\right)
\end{eqnarray*}



\section{Deactivation Layer Distribution}
%\subsubsection{Mean and Variance}
The mean of the deactivation layer is:
\begin{equation}
    \mu_w = \frac{s^\gamma}{\Gamma(a)}\Gamma( \gamma + a )
\label{eq:deact_mu}
\end{equation}

and the variance is:
\begin{equation}
    \sigma^2_w = \frac{s^{2\gamma}}{\Gamma(a)}\left( \Gamma(a + 2\gamma) - \frac{\Gamma(a+\gamma)^2}{\Gamma(a)}\right)
\label{eq:deact_sigma}
\end{equation}





% Newer deactivation that does not really work, deact with offset, dont know what the
% rate of convergence is, reverted back to original unoffset version
\section{Deactivation Distribution Mean and Variance}
\label{app:deact_mean_var}
We first derive the equation for obtaining the $n^{th}$ moment of a random variable $X$ with the deactivation distribution $w(x)$ in Thm. \ref{thm:deact_pdf}, which we denote as $\mathbb{E}[X^n]$:
\begin{eqnarray*}
\mathbb{E}[X^n] & = & \int^\infty_0 \frac{e^{\epsilon/s}}{\gamma\Gamma(a)s^a}\left(\sum^\infty_{k=0} \binom{a-1}{k}x^{\frac{a - 1}{\gamma}-k}(-\epsilon)^k\right) \times \\
& &\exp\left(-\frac{x^{1/\gamma}}{s}\right) x^n dx \\
&  =& \frac{e^{\epsilon/s}}{\gamma\Gamma(a)s^a} \sum^\infty_{k=0} \binom{a-1}{k}(-1)\epsilon^k \times \\
&& \int^\infty_0 x^{\frac{a}{\gamma}-k-1+n}\exp\left( - \frac{x^{1/\gamma}}{s}\right)\; dx
\end{eqnarray*}
We now evaluate the integral inside the sum in the above equation by performing change of variables with $y = x^{1/\gamma}/s$ so $dy/dx = (1/(\gamma s))x^{1/\gamma - 1}$ and $w(0) = 0$, resulting in the integral:
\begin{eqnarray*}
&&\int^\infty_0 x^{\frac{a}{\gamma}-k-1+n}\exp\left( - \frac{x^{1/\gamma}}{s}\right)\; dx \\& = & \int^\infty_0 (sy)^{a - \gamma(k+1-n)}e^{-y}\gamma s(sy)^{\gamma - 1}\; dy \\
& = & \gamma s^{a-\gamma(k-n)}\int^\infty_0y^{a + \gamma(n-k)-1}e^{-y}\; dy \\
& = &\gamma s^{a-\gamma(k-n)}\Gamma( a + \gamma(n-k) )
\end{eqnarray*}
Substituting the above result back into the moment equation gives:
\begin{eqnarray}
\mathbb{E}[X^n] &= & \frac{e^{\epsilon/s}}{\gamma\Gamma(a)s^a} \sum^\infty_{k=0} \binom{a-1}{k}(-\epsilon)^k \times \nonumber \\
&& \gamma s^{a-\gamma(k-n)}\Gamma( a + \gamma(n-k) ) \nonumber \\
& =& \frac{e^{\epsilon/s}}{\Gamma(a)} \sum^\infty_{k=0} \binom{a-1}{k}\frac{(-\epsilon)^k \Gamma( a + \gamma(n-k) ) }{s^{\gamma(k-n)}}
\label{eq:deact_mom}
\end{eqnarray}

Using the above equation for $\mathbb{E}[X^n]$, we can immediately obtain the expression for the mean of $w(x)$, denoted as $\mu_w$, by setting $n$ to 1:
\[
\mu_w = \frac{e^{\epsilon/s}}{\Gamma(a)} \sum^\infty_{k=0} \binom{a-1}{k}\frac{(-\epsilon)^k \Gamma( a + \gamma(1-k) ) }{s^{\gamma(k-1)}}
\]

For practical purposes, we can obtain an approximation of $\mu_w$ to order $O(\epsilon^{n+1})$ by using only the first $n$ terms in the sum of $\mu_w$ to get:
\begin{equation}
\mu_w \approx \frac{e^{\epsilon/s}}{\Gamma(a)} \sum^n_{k=0} \binom{a-1}{k}\frac{(-\epsilon)^k \Gamma( a + \gamma(1-k) ) }{s^{\gamma(k-1)}} %+ O(\epsilon^{n+1})
\label{eq:deact_mean_approx_appendix}
\end{equation}

To find the variance, we first find the second moment (denoting the random variable as $X_w$). This is achieved by using Eq. \ref{eq:deact_mom} and setting $n=2$ to get:
\begin{eqnarray*}
\mathbb{E}[X_w^2] & = & \frac{e^{\epsilon/s}}{\Gamma(a)} \sum^\infty_{k=0} \binom{a-1}{k}\frac{(-\epsilon)^k \Gamma( a + \gamma(2-k) ) }{s^{\gamma(k-2)}}
\end{eqnarray*}
As with the mean $\mu_w$, an approximation to order $O(\epsilon^{n+1})$ can be obtained when we restrict the infinite sum in $\mathbb{E}[X_w^2]$ to the first $n$ terms.
%
Finally, the variance (up to order $O(\epsilon^{n+1})$ is obtained using $\sigma_w^2 = \mathbb{E}[X_w^2] - \mu_w^2$ to give:
\[
\sigma_w^2 = \frac{e^{\epsilon/s}}{\Gamma(a)} \sum^n_{k=0} \binom{a-1}{k}\frac{(-\epsilon)^k \Gamma( a + \gamma(2-k) ) }{s^{\gamma(k-2)}} - \mu_w^2
\]
where $\mu_w$ also uses the approximation in Eq. \ref{eq:deact_mean_approx_appendix}.

% BACKUP tex for these results
% Eyepacs dataset results
\begin{figure}
    \centering
    \begin{tabular}{ccc}
    %Average Pool & Exp. Pool & KL-Div.\\
    \includegraphics[width=0.4\linewidth]{imgs/eyepacs_avpool.pdf} & \includegraphics[width=0.4\linewidth]{imgs/eyepacs_exppool.pdf} \\
    AvPl & ExpPl
    \end{tabular} 
    \caption{EyePACs Dataset predicted output node distributions (red and black curves) and observed underlying histograms. Black represents images with negative labels, whilst red represents images with positive labels.}
    \label{fig:eyepacs_out_distrib}
\end{figure}
\begin{figure}
    \centering
    \begin{tabular}{ccc}
         \includegraphics[width=0.33\linewidth]{imgs/cifar_kl.pdf}&  
         \includegraphics[width=0.33\linewidth]{imgs/flowers_kl.pdf} & 
         \includegraphics[width=0.33\linewidth]{imgs/eyepacs_kl.pdf} \\
         CIFAR10 & Flowers & EyePACs
    \end{tabular}
    \caption{Scatter plots of predicted (x-axis) against observed (y-axis) KL-divergence of the DNN output node.The green diagonal line on the right plot indicates when the predicted and observed KL divergence are equal. Blue circles indicate exponential activation, and black crosses indicate average pooling.}
    \label{fig:kl_plot}
\end{figure}


%%% Backup for CIFAR and floweres results figure text
\begin{figure*}
    \centering
    \begin{tabular}{ccccccccccc}
    AvPl&\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls0.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls1.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls2.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls3.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls4.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls5.pdf}
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls6.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls7.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls8.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls9.pdf} \\
    ExpPl&\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls0.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls1.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls2.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls3.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls4.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls5.pdf}
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls6.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls7.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls8.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls9.pdf} \\
    &C1 & C2 & C3 & C4 & C5 & C6 & C7 & C8 & C9 &C10
    \end{tabular}\\
    CIFAR10 Dataset\\
    \begin{tabular}{cccccc}
    AvPl&\includegraphics[align=c, width=0.15\linewidth]{flower_imgs/flower_daisy_avp.pdf} &
          \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_dan_avp.pdf}  
         & \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_rose_avp.pdf} & 
         \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flowers_sunflower.pdf} & 
         \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_tulip_avp.pdf} \\
         ExpPl &\includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_daisy_exp.pdf} 
         & \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_dan_exp.pdf}  
         & \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_rose_exp.pdf} & 
         \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_sunflower_exp.pdf} & 
         \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_tulip_exp.pdf} \\
          &Daisy & Dandl. & Rose & SunFlw. & Tulip
    \end{tabular} \\
    Flowers Dataset
    
    \caption{Examples of predicted output node distributions (red and black curves) and observed underlying histograms. Black represents images with negative labels, whilst red represents images with positive labels.}
    \label{fig:cifar_flowers_out_distrib}
\end{figure*}




\subsection*{Instance level retrieval of landmarks}
We develop and validate our proposed algorithm for image retrieval task. A baseline ResNet101 model is used, with activation pooling, trained with Arcface loss on Google landmarks retrieval v2 dataset. We evaluate the trained CNN on independent landmark retrieval datasets, Revisited Oxford ($R$Oxf) and Revisited Paris ($R$Par), using medium and hard setups referred as $R$Oxf$M$, $R$Par$M$, $R$Oxf$H$ and $R$Par$H$. 

It can be observed from Table \ref{MobileNettab} the our Activation CNN performs significantly better that the state-of-the-art on all four benchmarks.

\begin{table}[htbp]
\caption{Retrieval accuracy for three CNNs on retrieval datasets}
\label{MobileNettab}
\resizebox{\columnwidth}{!}{\begin{tabular}{|l|c|c|c|c|}
\hline & $R$Oxf$M$ & $R$Oxf$H$ & $R$Par$M$ & $R$Par$H$ \\ \hline \hline
Average pooling CNN &75.9  &55.2  &87.1 &73.9\\ \hline
ResNet101+ArcFace \cite{weyand2020google} &76.2 &55.6 & 87.3 &74.2 \\ \hline
Activation CNN &\bf{77.4}  &\bf{58.5} &\bf{88.3} &\bf{76.5}  \\ \hline

\end{tabular}}
\end{table}


==> contents_backup1.tex <==
% introduction comes here

\section{Introduction}
In recent years, deep neural networks (DNN) have shown excellent performance across a wide range of tasks, for example, image classification and retrieval.
% TODO - we want some citations here
It have become increasingly common for DNNs to use aggregation processes such as global average pooling in order to combine spatial semantic information into a compact deep global descriptor. 
% TODO - some DNNs that use aggregations??
%The use global aggregation methods has the advantage of making the DNN agnostic to the input image resolution. 
It was found in \cite{HusainPAMI} that the retrieval or classification performance of DNNs correlates strongly with an increase in the KL divergence of its outputs. Therefore, knowledge of how the KL divergence is theoretically related to earlier layers of a DNN will provide valuable knowledge into further improving the performance of existing DNNs. This in turn requires knowledge of the statistical distribution of different layers in DNNs.

\section{Related Work}
%In order to better understand and thus improve the performance of DNNs, an understanding of their probabilistic nature is beneficial. 
The theoretical understanding of the statistics of layers in DNN is currently an active area of research.
The connection between Gaussian Processes (GP) and a single fully connected layer of infinite neurons was initially established by Neal \cite{nealthesis}. 
Recently, the link between Gaussian Processes and neural networks with multiple hidden layers was shown by Lee et al. \cite{lee18} and Mathews et al. \cite{matthews2018gaussian}. This was further extended to cover deep nets with convolutional layers by Novak et al. \cite{Novak19}. However, the validity of the above work rests on the assumption of infinite channels and hidden units. Unfortunately, practical DNNs in use at present contain finite hidden units and convolutional channels. As such, it is still unclear what distributions outputs of convolutional layers in DNNs will take. 
% TODO - what does our work do to tackle the above issue?

% variational learning papers

% neurocomputing references to review and add - but the basic comment is as follows: each of the following work on activation functions attempt to smooth the discontinuity present at x = 0. However, the non-linear transformation is applied at x < 0. The linear function is still used for x >= 0, meaning that no amplification of the neuron outputs is performed. Our work does the opposite, in that we use non-linear transformation amplify the results in a non-linear manner.

% IMPORTANT TODO - emphasise that the application of our method is not to perform KL loss optimisation, but KL *maximisation* of distributions between different classes. Existing uses of KL divergence is to attempt to minimise the "distance" between the data/problem distribution and predicted distribution (from the DNN). In conventional DNNs, this is achieved by treating the value of a DNN output node as a probability (which is true when softmax is used) and comparing it with the probability set using the label. Knowledge of the underlying distributions of the different layers cannot be used. We optimise directly the distributions of the output nodes from the entire dataset instead of batches or individual samples.
% Question - is this the same thing?! Differences between distribution optimisation vs KL-divergence loss in a batch-learning situation.
\subsection{Contributions and Overview}
% -  
In the next section, we describe and review existing DNN architectures that employ aggregation methods.
The later sections contain the contributions of this paper which we list as follows: 
\begin{itemize}
\item We propose a non-linear aggregation process that involves initial exponential amplification, followed by aggregation and finally deactivation (Section \ref{sec:nonlin_act_agg}). 
\item We carry out a theoretical study how the distribution of information changes across the aggregation layers as illustrated in Fig. \ref{fig:nn_overview} (Section \ref{sec:agg_blocks}), where we propose a novel mixed distribution for modelling the outputs of the last convolutional layer.
%Here, we first propose a novel mixed distribution for modelling the outputs of the last convolutional layer (Section \ref{sec:agg_blocks}). Here, we derive the distributions for each layer involved in the aggregation process. 
\item We are able to derive the distribution and statistics of each layer in the aggregation process. 
\item We also propose a formulation for analytically predicting the KL-divergence of the outputs of a DNN based solely on the last convolutional layer distributions.
%These are linked with the classification layer, giving us a distribution for the output nodes of the DNN (Section \ref{sec:class_kl}.
%We then apply this knowledge on analytically predicting the KL divergence of the outputs of DNNs based solely on the last convolutional layer observed distributions.
\item We propose a novel method for optimising the KL-divergence of a DNN in terms of its underlying probability distributions instead of the commonly used sample-based methods (such as batches of examples in stochastic gradient descent).
\end{itemize}
We perform experiments and show that our mathematical formulations can be used to accurately predict the distributions for layers involved in the aggregation of deep features (Section \ref{sec:exp}), before concluding in Section \ref{sec:conclusions}.

\begin{figure*}[t!]
\begin{center}
\includegraphics[width = 1\linewidth]{ARCH_cvpr2.pdf} 
\end{center}
\caption{An overview of how the distribution of values from the last convolutional layer (for images of a specific label) is transformed by a nonlinear activation layer, followed by the pooling layer, deactivation layer, before being combined together into an output distribution.}
\label{fig:nn_overview}
\end{figure*}

\section{Aggregation DNN Classifiers}
% Question - should this even be a section??? 
In this paper, we consider DNN architectures that have the following structure: base-network $\rightarrow$ aggregation block $\rightarrow$ fully connected classification layer.

The base network typically consists of a sequence of convolutional blocks, and can be somewhat shallow (AlexNet \cite{krizhevsky2012imagenet}, VGG \cite{simonyan2014very}) to very deep (ResNet101 \cite{resnet}, Xception \cite{Xception}). 
The final convolutional layer then produces an output tensor that is passed to the aggregation block, where features are aggregated together to form compact global image signature. The popular feature aggregation methods are Global max pooling (GMP) \cite{MAC}, Global average pooling (GAP) \cite{GAP}, NetVLAD \cite{NetVLAD}, Generalized mean pooling (GEMP) \cite{GEM}, Region of interest pooling (ROIP) \cite{ROIP} and REMAP \cite{REMAP}. This global descriptor is then passed to a fully connected classification layer for producing the output result.

Our work is concerned with understanding the statistics of the aggregation block and how information is transformed within it. We also consider the case where the final convolutional layer features are amplified non-linearly before and after the aggregation process.

\section{Non-linear Activated Aggregation}
\label{sec:nonlin_act_agg}
% TODO - some information on the non-linear activation
Let $F$ be the number of filters in the last convolutional layer. Given an input image, the last convolutional layer will produce an output tensor $\mathbf{T}$ of size $W\times H \times F$ pixels. The elements of $\mathbf{T}$ is denoted as $T_{ijk}$ where $i \in \{1,2,...,W\}$, $j \in \{1,2,...,H\}$ and $k \in \{1,2,...,F\}$. Additionally, the total number of output pixels from each filter is written as $R = WH$.

% describe the non-linearly activated version (aka standard average pooling)
In many popular DNNs, an aggregation of the last convolutional layer featurs are performed, typically using global average pooling (GAP), giving a $F$-dimensional ``global descriptor'' vector $\mathbf{d} = (d_1,d_2....d_F)$ of the input image, where its elements are:
\begin{equation}
    d_f = \frac{1}{R} \sum^N_i\sum^N_j T_{ijf}
\end{equation}

The vector $\mathbf{g}$ is given as input to a fully connected layer for classification.

In our work, we also consider the use of a non-linear transformation {\em before} aggregation using GAP. Specifically, each element of the last convolutional layer tensor $\mathbf{T}$ is transformed using the scaled exponential function:
\begin{equation}
g(x) = \alpha ( \exp(\beta x ) - 1 )
\label{eq:scaled_exp_trans}
\end{equation}

The result is then passed through the GAP operation to produce an exponentially amplified global descriptor $\mathbf{e} = (e_1,e_2,...,e_F)$, where the elements are:
\[
e_f = \frac{1}{R} \sum^N_i\sum^N_j g( T_{ijf} )
\]

% describe the deactivation
The exponential amplification of tensor elements can produce values that are very large. To overcome this issue, a ``deactivation'' process is performed by raising the amplified global descriptor to a small power $\gamma$ (less than 1): 
\begin{equation}
    s(x) = x^\gamma
\end{equation}

This produces the following non-linearly aggregated descriptor $\mathbf{e'} = (e'_1, e'_2,...,e'_F)$ that is used for classification, where:
\[
e'_f = s( e_f )
\]

\section{Statistics of Aggregation Blocks} \label{sec:agg_blocks}

In this section, we propose a novel formulation for the statistics of different operations in an aggregation block. 
This allows us to conduct important theoretical study on the way distribution information changes as they pass through different layers in an aggregation block. 
This will later provide an important link between features of the last convolutional layer and the KL-divergence of two classes at the output layer.
We start by proposing a suitable statistical model that describes the distribution of output values of the last convolutional layer of a DNN.

\subsection{Last Convolutional Layer Mixed-Distribution}
\label{sec:last_conv_mix_distrib}
% In this section, we conduct a study of how output values of the last convolutional layer filters are distributed, particularly when ReLU is used as an activation function.
In this section, propose a probabilistic model capturing how the last convolutional layer outputs are distributed, particularly when ReLU is used as an activation function.

{\em TODO: IMPORTANT POINT TO MAKE: - Common assumption that the input will be Gaussian distributed is NOT valid here, since they are immediately taken from a ReLU process. The subsequent amplification process does not involve any combination of these random variables, and the aggregation tend to be based on the receptive field size which is also small, so Gaussian assumption may not yield a sufficiently accurate approximation, we have a more accurate one. The result is also true for the de-activation stage.}
%We describe a probability distribution that was found to fit the output values of convolutional layers with ReLU activations.
To this end, it was found that output values greater than 0 can be modelled well by a Gamma distribution:
 \begin{equation}
     f_\Gamma(x) = \frac{1}{\Gamma(a)s^a}x^{a-1}\exp(-x/s)
     \label{eq:gamma_pdf}
 \end{equation}
where $a$ and $s$ are the shape and scale parameters respectively. Additionally, the $\Gamma(z)$ denotes the complex valued Gamma function, a continuous analogue of the factorial function, which we use extensively in this paper, and is defined as:
\[
 \Gamma(z) = \int^\infty_0 x^{z-1}e^{-x} dx
\]

%The Gamma distribution brings a number of beneficial properties:  
% {\em IMPORTANT POINT: Why GAMMA DISTRIBUTION for positive values?? Because it is easy to deal with, captures exponential, skewed data, and towards a gaussian }
% {\em ALSO IMPORTANT: Gamma distribution makes sense for modelling the positive values, since ReLUed activations will take non-negative values.}
% 
However, the use of ReLU also has the effect of concentrating all the mass of the pdf at 0 and negative values of $x$ to a single point of $x = 0$. Thus, in order to capture such a behaviour, we will use the following mixed probability distribution defined in the range $[0,\infty)$:
\begin{equation}
f(x) = \left\{ \begin{array}{cc}
     p &, \textrm{if}\;\; x = 0 \\
     (1-p)\frac{1}{\Gamma(a)s^a}x^{a-1}\exp(-x/s)& , \textrm{if}\;\; x > 0
\end{array}\right.
\label{eq:zero_gamma_pdf}
\end{equation}
where $p$ is the probability of values less or equal to 0. The Gamma distribution used for values $x > 0$ with a location parameter of 0 was found to give a good fit to observed data whilst being simpler to work with. 

\subsubsection{Mean and Variance}
To use this distribution, it is important that its mean and variance is known. To start, let $X$ be a random variable with pdf of $f(x)$ (Eq. \ref{eq:zero_gamma_pdf}).
We find that the mean of $X$ is the weighted mean of the Gamma distributed component:
\begin{eqnarray}
\mu_f & = & \mathbb{E}[X] %\nonumber \\
%& = & 
 = \int^\infty_0 f(x)x dx \nonumber\\
& = & \int^\infty_0 (1-p)\frac{1}{\Gamma(a)s^a}x^{a-1}\exp(-x/s)x dx \nonumber \\
& = & (1-p)as 
\label{eq:zero_gamma_mean}
\end{eqnarray}
The last line above uses the fact that the mean of a Gamma distribution is $as$. Next, to find the variance, denoted as $\sigma^2$, we first note that:
\begin{equation}
\sigma^2 = \mathbb{E}[X^2] - (\mathbb{E}[X])^2
\label{eq:gen_var}
\end{equation}

To proceed, we will need to find the second moment of $X$ which is defined as:
\begin{eqnarray}
\mathbb{E}[X^2] & = & \int^\infty_0 f(x) x^2 dx \nonumber \\
& = & \int^\infty_0 (1-p)\frac{1}{\Gamma(a)s^a}x^{a-1}\exp(-x/s)x^2 dx \nonumber \\
& = & (1-p)a(a+1)s^2
\label{eq:zero_gamma_2nd_mom}
\end{eqnarray}
The last equation above is obtained by using moment generating functions on the Gamma distribution (details of the derivation in Appendix \ref{app:mix_gamma_scnd_mnt_deriv}). Then, by substituting Eq. \ref{eq:zero_gamma_2nd_mom} and Eq. \ref{eq:zero_gamma_mean} into Eq. \ref{eq:gen_var}, we have the variance as:
\begin{eqnarray}
Var(X) & = & (1-p)a(a+1)s^2 - (1-p)^2a^2s^2 \nonumber \\
& = & (1-p)as^2( a - (1-p)a ) \nonumber \\
& = & (1-p)as^2(1+ap)
\end{eqnarray}

%\subsection{Mixed One-ExpGamma Distribution}
\subsection{Distribution of Non-linear Activation}
We will now describe how a non-linear activation on mixed-Gamma tensor values will transform its distribution. In particular, we consider the scaled exponential transform: $g(x) = \alpha( \exp(\beta x ) - 1$ (Eq. \ref{eq:scaled_exp_trans}).

We have seen in Section \ref{sec:last_conv_mix_distrib} how the distribution of each last convolutional layer filter output is modelled as a mixture of a discrete point distribution at 0 and Gamma distribution for positive values. Consequently, if this zero-Gamma mixed distribution was exponentiated, the result will be a new mixed distribution, with a discrete component again at 0 and an exponentiated Gamma distribution $h(x)$ (which we describe next in Section \ref{sec:exp_gamma}) for all values greater than 0. In other words, we have the new distribution $h_m$, %(subscript $m$ for ``mixed''), 
which we call the ``Zero-ExpGamma'' distribution and is defined for $x \geq 0$:
\begin{eqnarray}
h_m(x) = \left\{
\begin{array}{cc}
     p & ,\textrm{if}\;\; x = 1 \\
     (1-p)h(x) & ,\textrm{if}\;\; x > 1
\end{array}
\right.
\label{eq:zero_exp_gamma_pdf}
\end{eqnarray}

\subsubsection{Exponentiated Gamma Distributions}
\label{sec:exp_gamma}
We start by determining the distribution for an exponentially transformed Gamma distribution. So, suppose a random variable $X$ follows the Gamma distribution described in Eq. \ref{eq:gamma_pdf}. We would like to know what the distribution of this random variable when it is exponentially transformed.
\begin{theorem}
Let $X$ be a random variable with distribution $f_\Gamma(x)$ in Eq. \ref{eq:gamma_pdf}. Let $g(x) = \alpha( \exp(\beta x) - 1)$ with $\alpha, \beta \in \mathbb{R}$, then $g(X)$ follows the following distribution:
\[
h(x) = \frac{1}{\Gamma(a)\beta^as^a}(\ln (1+x/\alpha))^{a-1}(1+x/\alpha)^{-\left(\frac{\beta s +1}{\beta s}\right)}
\]
\label{thm:exp_gamma}
\end{theorem}
The proof of this theorem is a straightforward application of the transformations of variables method commonly used to determine the distributions of transformed random variables. It requires that the transformation function has a differentiable inverse, which is the case here. Details of the proof can be found in Appendix \ref{app:exp_gamma_pdf}.
%\subsection{Mean and Variance}
%The mean and variance of the exponentiated Gamma distribution is important for later use, especially in predicting the distributions of the output layer distributions. Thus, if $X$ is a random variable following the distribution of $h(x)$ of Theorem \ref{thm:exp_gamma}, 
The mean of $h(x)$ is:
\[
%\mathbb{E}[X] 
\mu_h = \alpha\left(\frac{1}{(1- \beta s)^a} - 1\right)
\]
The variance of this distribution is:
\begin{equation*}
%Var(X) 
\sigma^2_h = \frac{\alpha^2}{(1-2\beta s)^a} - \frac{\alpha^2}{(1-\beta s)^{2a}}
\end{equation*}
The derivation of the above mean and variance can be found in Appendix \ref{app:zero_expgamma_meanvar}. 
% TODO - describe some simulations to verify this , Done, describe this

\subsubsection{Zero-ExpGamma Mean and Variance}
The mean and variance of the mixed zero-ExpGamma distribution can be obtained in a similar manner to that of the zero-Gamma distribution. 
The mean of $h_m(x)$ is:
%Let $X_m$ be the random variable with distribution $h_m(x)$. The mean of $X_m$ is then:
\begin{eqnarray}
\mu_{m} %& = & \mathbb{E}[X_m] \nonumber\\
& = & \int^\infty_0 h_m(x)x dx %\nonumber\\
 =  \int^\infty_0 (1-p)h(x) x dx \nonumber\\
& = & (1-p)\mu_h = \alpha(1-p)\left(\frac{1}{(1 - \beta s)^a} - 1\right)
\label{eq:zero_expgamma_mean}
\end{eqnarray}

The variance of $h_m(x)$ is found in the same manner as the previous distributions, by finding the second moment and subtracting the squared mean from it. The result is (derivation in Appendix \ref{app:zero_expgamma_var}):
\begin{eqnarray}
\sigma_m^2& = & \alpha^2(1-p)\left[ \frac{1}{(1-2\beta s)^a} - \frac{1-p}{(1-\beta s)^{2a}} - \right. \nonumber \\
&& \left. \frac{2p}{(1-\beta s)^a} + p \right]
\label{eq:zero_expgamma_var}
\end{eqnarray}
%\begin{equation}
%    \sigma^2_m = p(1-p) + \frac{1-p}{(1-2\beta s)^a} - \frac{(1-p)2p}{(1 - \beta s)^a} - \frac{(1-p)^2}{(1-\beta s)^{2a}}
%\end{equation}

\subsubsection{Powered Zero-Gamma Distribution}
% describe the distribution here
In this section, we will consider the effect of performing activation by raising the tensor values to some fixed power (that is learnable). This form of activation has been used in existing work on image retrieval \cite{GEM}. 

% mean and variance here
%\subsection{Sum of $N$ Zero-Gamma Distributed Random Variables}
\subsection{Probability Distribution of GAP Features}
We are now in position to determine the distribution of global average pooled features. We assume that the ``pixels'' in the output convolutional image of each filter will follow either the zero-gamma or zero-ExpGamma distribution (depending on whether non-linear activation was used). 
%We further assume that they are independent. 
% TODO - 
Importantly, we have found that the convolutional image pixels are correlated both within the same filter and between different filters. This will need to be considered when we are calculating the variance of each filter.

The convolutional output of a particular filter can be modelled as a collection of $R$ (i.e. total pixels in convolutional image) dependent random variables. The GAP operation has the effect of taking the average (i.e. weighted sum) of $R$ random variables.
%of a sum of random variables all with the zero-gamma distribution. This will be useful for determining the distributions of global pooling layers, for our case, the global average pooling layer.

We denote the above $R$ random variables as $X_1,X_2,...,X_R$. The  distribution of these random variables can either be Eq. \ref{eq:zero_gamma_pdf} or Eq. \ref{eq:zero_exp_gamma_pdf}. As such, we will denote their respective means and variance using $\mu_*$ and $\sigma^2_*$, where $* \in \{f,m\}$ is a placeholder for whether exponential activation is used ($* = m$) or not ($* = f$). 
The GAP operation will produce a new random variable, $X_S$, that is the average of $X_1,X_2...,X_R$: 
%$X_S = (1/R)(X_1 + X_2 + ... + X_R)$.
\[
X_S = \frac{1}{R}\sum^R_{i=1}X_i
\]

The exact distribution can be very complicated, particularly for the case of the zero-ExpGamma case. We will later describe (Section \ref{sec:gap_pdf_approx}) how it is possible to approximate the ``GAP feature'' distribution as a Gamma distribution. However, to determine the shape and scale parameter of this distribution we will need the mean and variance of $X_S$. We start with the mean, denoted as $\mu_{X_S}$, which is obtained using the linearity property of the expectation operator:
%The mean is straightforward to work out:
\begin{eqnarray}
\mu_{X_S} & = & \mathbb{E}[X_S] 
%& = & 
=\mathbb{E}\left[\frac{1}{R}\sum^R_{i=1}X_i \right]\nonumber \\
& = & \frac{1}{R} \sum^R_{i=1} \mathbb{E}[X_i] %\nonumber \\
%& = & 
%= \frac{1}{N}N(1-p)as \nonumber \\
%& = & (1-p)as
= \mu_*
\label{eq:gapsum_mean}
\end{eqnarray}
In other words, the mean is unchanged by the averaging operation. 

\subsubsection{GAP Feature Variance Prediction}
\label{sec:gap_feat_var_pred}
Since the pixels of each filters are correlated, the variance of the GAP distribution will also depend on the covariance matrix of the convolutional pixels of a filter. Unfortunately, determining the exact covariance matrix of a sum of correlated R.V.s will require knowing their joint distribution. We avoid directly tackling this issue by using a 2nd order Taylor approximation of the covariance matrix. We have found that this order is sufficient to provide an accurate estimation of the covariance matrix. This has an advantage of not requiring us to explicitly know the joint distribution of all pixels in a convolutional image for a specific filter.

To start, let the elements of the $R\times R$ covariance matrix between the random variables $X_1,X_2,...,X_R$ be denoted as $Cov_S(i,j)$, with $i,j\in\{1,2,...,R\}$ where:
\begin{eqnarray}
Cov_S(i,j) & = & \mathbb{E}[(X_i - \mu_{X_i})(X_j - \mu_{X_j})] \nonumber \\
&=& \mathbb{E}[X_iX_j] - \mu_{X_i}\mu_{X_j}
\label{eq:gap_cov_mat}
\end{eqnarray}

Our task now is to calculate $\mathbb{E}[X_iX_j]$. 
Suppose that $X_i$ is the result of the non-linear activation of the random variable $W_i$ (i.e. $W_i$ is some pixel of the last convolutional layer) using the function $g(x)$, that is: $X_i = g(W_i)$. Next, the 2nd order Taylor expansion of $g(x)$ at $x = 0$ gives $g(x) \approx g(0) + g'(0)x + g''(0)x^2/2$. 
Inserting this expansion into $\mathbb{E}[X_iX_j]$ gives:
\begin{eqnarray}
\mathbb{E}[X_iX_j] & = & \mathbb{E}[g(W_i)g(W_j)] \\
& \approx & \mathbb{E}\left[\left(g(0) + g'(0)W_i + \frac{g''(0)W_j^2}{2}\right)\times \right.\nonumber\\
&&\left. \left(g(0) + g'(0)W_j + \frac{g''(0)W_j^2}{2}\right)\right] \nonumber\\
& = & \mathbb{E}\left[g^2(0) + A(W_i + W_j) + BW_iW_j + \right.\nonumber\\
&& \left.C(W_i^2W_j + W_iW_j^2) + DW_i^2W_j^2\right] \nonumber\\
& = & g^2(0) + A(\mathbb{E}[W_i] + \mathbb{E}[W_j]) + B\mathbb{E}[W_iW_j] + \nonumber\\
&& C(\mathbb{E}[W_i^2W_j] + \mathbb{E}[W_iW_j^2] ) + D\mathbb{E}[W_i^2W_j^2]
\label{eq:exp_xi_xj}
\end{eqnarray}
with constants $A = g(0)g'(0)$, $B = (g'(0))^2$, $C = g'(0)g''(0)/2$ and $D = g''(0)^2/4$. 

We are now faced with the issue of calculating the expectations: $\mathbb{E}[W_i^a,W_j^b]$ where $a,b \in {0,1,2}$. We can achieve this {\em without} the need for knowing what the joint distribution between $W_i$ and $W_j$ is by using the relationship: $\mathbb{E}[W_i^aW_j^b] = Cov(W_i^a,W_j^b) - \mu_{W_i}\mu_{W_j}$. Here, the covariance matrix $Cov(W_i^a,W_j^b)$ and means $\mu_{W_i},\mu_{W_j}$ can all be directly computed using the data from the last convolutional layer outputs. Since we will be using the approximation of $\mathbb{E}[X_iX_j]$, we should also use the approximation of $\mu_{X_i}$ and $\mu_{X_j}$ too, where:
\begin{equation}
\mu_{X_i} \approx g(0) + g'(0)W_i \frac{g''(0)}{2}W_i^2
\label{eq:gap_mu_approx}
\end{equation}
with $\mu_{X_j}$ obtained in a similar manner.

Finally, plugging the approximations of $\mathbf{E}[X_iX_j]$ (Eq. \ref{eq:exp_xi_xj} and $\mu_{X_i}, \mu_{X_j}$ (Eq. \ref{eq:gap_mu_approx}) back into Eq. \ref{eq:gap_cov_mat} will give us an estimate of the $R\times R$ covariance matrix of different pixels in a particular filter.

% give an example for the case where g(x) is the exponential activation function

We can now calculate the variance. This is the sum of the variances of $X_i$ scaled by a factor of $1/R$, with a correction factor based on the covariance matrix added in:
\begin{eqnarray}
\sigma^2_{X_S} &=& Var(X_S) \\
&= & Var\left(\frac{1}{R}\sum^R_{i=1}X_i \right) + \sum^R_{\substack{i,j=1\\ i\neq j}}Cov_S(i,j) \nonumber \\
& = & \sum^R_{i=1}\frac{1}{R^2} Var(X_i) + \sum^R_{\substack{i,j=1\\ i\neq j}}Cov_S(i,j) \\
%& = & 
& = &\frac{1}{R}\sigma^2_* + + \sum^R_{\substack{i,j=1\\ i\neq j}}Cov_S(i,j)
%& = & \frac{1}{N}(1-p)as^2(1+ap)
\label{eq:gapsum_var}
\end{eqnarray}

\subsubsection{GAP Feature Distribution Approximation}
\label{sec:gap_pdf_approx}
We now find the distribution of $X_S$. 
First, the zero values of $X_S$ will have a probability of $p^N$. In the case for non-zero positive values, when we are considering only average pooled aggregation, we find that the sum of a set of identically Gamma distributed random variables will produce another Gamma distributed random variable. Interestingly, we find that the Gamma distribution also provides a good approximation when we are considering the sum of exponentiated Gamma distributions. In fact, the higher the resolution of the convolutional image, the better the approximation.
Thus, in both cases, we will assume that the non-zero values of $X_S$ will follow a Gamma distribution. 

To obtain its shape and scale parameters, $a_S$ and $s_S$ respectively,
we will use $\mu_{X_S}$ (Eq. \ref{eq:gapsum_mean}) and $\sigma^2_{X_S}$(Eq. \ref{eq:gapsum_var}).
%we note that for a Gamma distribution, if its mean and variance, $\mu_G, \sigma^2_G$ say, is known, it is possible to recover the shape and scale parameters from them. 
Next, we find that $\mu_{X_S} = a_Ss_S$ and $\sigma^2_{X_S} = a_Ss^2_S$. Thus, dividing the variance with the mean gives the scale parameter and substituting $s$ into the first equation and rearranging gives $a_S$:
\[
s_S = \frac{\sigma_{X_S}^2}{\mu_{X_S}},\;\;\textrm{and}\;\;a_S = \frac{\mu_{X_S}^2}{\sigma_{X_S}^2}
\]

%\begin{eqnarray}
%s_S & = & \frac{\sigma^2_G}{\mu_G} \nonumber \\
%& = & \frac{(1-p)a_Ss_S^2(1+a_Sp)}{(1-p)a_Ss_S} \nonumber \\
%& = & s_S(1+a_Sp)
%\end{eqnarray}
%
%We can now find the shape parameter, $a_S$ as follows:
%\begin{eqnarray}
%a_S & =& \frac{\mu_G}{s_S} \nonumber \\
%& = & \frac{(1-p)^2a_S^2s_S^2}{(1-p)a_Ss_S^2(1+a_Sp)}\nonumber \\
% & = & \frac{(1-p)a_S}{1 + a_Sp}
%\end{eqnarray}

Thus, each dimension of the GAP feature vector will have the following distribution:
%for the sum of $N$ identically zero-Gamma distributed random variables is:
\[
f_S(x) = \left\{
\begin{array}{cc}
     p^N &, \textrm{if}\;\; x = 0  \\
     \frac{1-p^N}{\Gamma(a_S)s_S^{a_S}}x^{a_S -1}\exp(-x/s_S)& , \textrm{if}\;\; x > 0 
\end{array}
\right.
\]
At this point, we note that $p^N$ will be extremely small (since $N$ tends to be tens to hundreds for typical convolutional image sizes), and we will take it to be 0, and $1-p^N$ will be taken to be 1. Consequently, we can ignore the $x=0$ branch of the above distribution, giving a simpler form of:
\begin{equation}
    f_S(x) = \frac{1}{\Gamma(a_S)s_S^{a_S}}x^{a_S-1}\exp(-x/s_S)
\label{eq:gap_pdf}
\end{equation}
\subsection{GAP Features Covariance Matrix}
In order to predict the variances of DNN layers after the GAP layer, we will require the covariance matrix of the GAP features. In this section, we describe an approximation of this covariance matrix using a 2nd order Taylor expansion. To start, let the number of GAP features to be $N$, giving an $N\times N$ GAP feature covariance matrix. Let the random variable of each GAP feature be denoted to be $Y_i$ where $i = 1,2,...,N$. Then, each GAP feature, $Y_i$ can be written as the average of $R$ associated convolutional pixels that have been transformed by some function $g(x)$\footnote{If no non-linear activation was performed, we simply set $g(x) = x$.}, denoted as $g(X_{i,1}),g(X_{i,2}),...,g(X_{i,R})$. Thus, the $i^{th}$ GAP feature random variable can be written as: 
\[
Y_i = \frac{1}{R}\sum^R_{k=1} g\left(X_{i,k}\right)
\]
The covariance between two GAP features, $Y_i$ and $Y_j$, say, is:
\begin{eqnarray}
Cov_G( i, j ) & = & \mathbb{E}[(Y_i - \mu_{Y_i})(Y_j - \mu_{Y_j})]\\ 
& = & \mathbb{E}\left[\left(\frac{1}{R}\sum^R_{k=1} g\left(X_{i,k}\right)- \mu_{Y_i}\right) \right.\times \nonumber \\
&& \left.\left(\frac{1}{R}\sum^R_{k=1} g\left(X_{j,k}\right)- \mu_{Y_j}\right) \right] \nonumber\\
&=& \frac{1}{R^2}\mathbb{E}\left[\left(\sum^R_{k=1}g(X_{i,k})\right) \left(\sum^R_{k=1}g(X_{j,k})\right)\right] - \nonumber\\
&&\mu_{Y_i}\mu_{Y_j} \nonumber\\
& = & \frac{1}{R^2}\mathbb{E}\left[\sum^R_{k=1}\sum^R_{l=1}g(X_{i,k})g(X_{j,l})\right] - \mu_{Y_i}\mu_{Y_j} \nonumber\\
& = & \frac{1}{R^2}\left(\sum^R_{k=1}\sum^R_{l=1}\mathbb{E}\left[g(X_{i,k})g(X_{j,l})\right]\right) - 
\mu_{Y_i}\mu_{Y_j}
\label{eq:gap_cov}
\end{eqnarray}

Our task is now to find an accurate enough estimate of $\mathbb{E}[g(X_{i,k})g(X_{j,l})]$. For this, we again perform a second order Taylor expansion on $g(x)$ around $x=0$, so that $g(x) \approx a + bx + cx^2$, where for conciseness, we have written the expansion coefficients as: $a = g(0), b = g'(0)$ and $c = g''(0)/2$. For more clarity, we will denote $U = X_{i,k}$ and $W = X_{j,l}$. This gives:
\begin{eqnarray*}
\mathbb{E}[g(U)g(W)] & \approx & \mathbb{E}\left[ (a + bU + cU^2)(a + bW + cW^2)
\right] \\
& = & \mathbb{E}\left[ a^2 + ab(U+W) + ac(U^2 + W^2) +\right. \\
&& \left. b^2UW + bc(U^2W + UW^2) + c^2U^2W^2 \right]\\
& = & a^2 + ab(\mathbb{E}[U]+\mathbb{E}[W]) + ac(\mathbb{E}[U^2] + \mathbb{E}[W^2]) + \\
&& b^2\mathbb{E}[UW] + bc(\mathbb{E}[U^2W] + \mathbb{E}[UW^2]) + \\ && c^2\mathbb{E}[U^2W^2]
\end{eqnarray*}
From the last equation above, we can see that a second order approximation of the GAP feature covariances can be obtained through first and second moments, as well as cross-covariances of the random variables of last convolutional layer output pixels. As such, they can be directly computed from a training set of last convolutional layer responses. The cross-covariances of the form: $\mathbb{E}[U^aW^b]$, with $a,b \in \{0,1,2\}$ can be computed in the similar manner as those used in the GAP feature variance prediction (Section \ref{sec:gap_feat_var_pred}).

\subsection{Deactivation Layer Distribution}
In the case where the non-linear exponential operator was used to amplify the tensor values before GAP, we find that the resulting values after GAP can potentially be very large. To address this issue, the deactivation layer is usually used. 
We will now describe the distribution of the deactivation layer.
\begin{theorem}
% TODO - FIX THE DISTRIBUTION! NOT CORRECT WITH +EPS ADDITION
Let $X$ be a random variable with distribution $f_S(x)$ in Eq. \ref{eq:gap_pdf}. Let $g(x) = (x+\epsilon)^\gamma$ with $\gamma \in \mathbb{R}$, where $\epsilon>0$ is a small positive real constant, then $g(X)$ follows the following distribution:
%\[
%w(x) = \frac{1}{\gamma\Gamma(a)s^a}x^{\frac{a-1}{\gamma}}\exp\left(-\frac{x^\gamma}{s}\right)
%\]
\[
w(x) = \frac{e^{\epsilon/s}}{\gamma\Gamma(a)s^a}\left(\sum^\infty_{k=0} \binom{a-1}{k}x^{\frac{a - 1}{\gamma}-k}(-\epsilon)^k\right) \exp\left(-\frac{x^{1/\gamma}}{s}\right)
\]

\label{thm:deact_pdf}
\end{theorem}
The proof of the above can be found in Appendix \ref{app:deact_pdf_proof}.

The mean  of the deactivation layer (up to order $O(\epsilon^{n+1})$) are respectively:
\begin{equation}
\mu_w = \frac{e^{\epsilon/s}}{\Gamma(a)} \sum^n_{k=0} \binom{a-1}{k}\frac{(-\epsilon)^k \Gamma( a + \gamma(1-k) ) }{s^{\gamma(k-1)}} %+ O(\epsilon^{n+1})
\label{eq:deact_mu}
\end{equation}
and the corresponding variance is:
\begin{equation}
\sigma_w^2 = \frac{e^{\epsilon/s}}{\Gamma(a)} \sum^n_{k=0} \binom{a-1}{k}\frac{(-\epsilon)^k \Gamma( a + \gamma(2-k) ) }{s^{\gamma(k-2)}} - \mu_w^2
\label{eq:deact_sigma}
\end{equation}

The above mean and variance derivations can be found in Appendix \ref{app:deact_mean_var}.

\subsubsection{Deactivation Feature Covariance}
In this section, we give an approximation of the covariance matrix for the $N$ deactivated GAP features. Thus, let $X,Y$ denote two random variables of two GAP features. In the case where our deactivation function is $g(x) = (x+\epsilon)^\gamma, \epsilon > 0$, we are seeking an approximation of $Cov( X^\gamma, Y^\gamma )$, which can be written as:
\begin{eqnarray}
Cov_D(X^\gamma, Y^\gamma) & = & \mathbb{E}[X^\gamma Y^\gamma] - \mathbb{E}[X^\gamma]\mathbb{E}[Y^\gamma]
\label{eq:deact_cov}
\end{eqnarray}
We have found that in this case, a first order Taylor approximation sufficed and has the advantage of only needing expectations that can be directly computed from training examples from the last convolutional layer outputs. Thus, taking the expansion of $g(x) = (x + \epsilon)^\gamma$ at $x = \epsilon$ gives us:
$g(x) \approx g(\epsilon) + \gamma(2\epsilon)^{\gamma - 1}(x-\epsilon)$, and for brevity, we will write $g(x) \approx c + dx$, with constants $d = \gamma(2\epsilon)^{\gamma - 1}, c = g(\epsilon)=(2 - d)\epsilon, $. 
First, the first order approximation for the mean of the deactivated random variable $X$ should be used:
\[
\mathbb{E}[X^\gamma] \approx c + d\mathbb{E}[X]
\]
where $\mathbb{E}[X]$ is the mean of the GAP feature associated with random variable $X$. In a similar manner, we can also obtain the approximation for $\mathbb{E}[Y]$.
Next, we can approximate the joint expectation $\mathbb{E}[X^\gamma Y^\gamma]$ as follows:
\begin{eqnarray*}
\mathbb{E}[X^\gamma Y^\gamma] & = & \mathbb{E}[(c + dX)(c + dY)] \\
& = & c^2 + cd( \mathbb{E}[X] + \mathbb{E}[Y] ) + d^2\mathbb{E}[XY]
\end{eqnarray*}
where $\mathbb{E}[XY]$ can be calculated using the covariance matrix from the GAP variables given in Eq. \ref{eq:gap_cov}, where suppose $X$ and $Y$ corresponds to the $i^{th}$ and $j^{th}$ GAP features respectively:
\[
\mathbb{E}[XY] = Cov_G( i, j ) - \mu_X\mu_Y
\]
and where $\mu_X, \mu_Y$ are the mean of the GAP feature random variables $X$ and $Y$ respectively.

\section{Classification KL-Divergence}.
\label{sec:class_kl}
% Pre-activation output nodes will have a distribution close to a normal distribution
In this section, we will determine the distribution of a DNN output node, and in the process mathematically linking it with the aggregation layer distributions. This gives us the important ability to analytically predict the KL divergence of the DNN output nodes from the convolutional layer outputs.  

\subsection{Output Layer PDF Approximation as Normal Distribution}
In this section, we will describe the distribution of values from a DNN output layer. Here, we assume that the GAP layer is immediately followed by a fully connected (FC) classification layer. We will also consider the distribution {\em pre-activation} (i.e. before the softmax or sigmoid activation).

The use of an FC layer after the GAP layer means that the elmenents of the GAP feature vector will be linearly combined together. Thus, if each element of the GAP feature is represented as a random variable following a distribution of the form $f_S(x)$ (Eq. \ref{eq:gap_pdf}), the output layer nodes can be represented by a linear combination of GAP random variables.

We typically find that the number of GAP features ($F$, the number of filters in the last convolutional layer) is typically high, ranging from hundreds to thousands. Thus, we can use the Central Limit theorem to approximate the distribution of a DNN output node as a Normal distribution. This is extremely convenient since we only need to know the mean and variance and covariance matrix of the GAP elements.
%This allows us to use the Central Limit Theorem, we can approximate the resulting linear combination of such Gamma distributed GAP features as a Normal distribution. 

%TODO - VERY IMPORTANT!! The text below is mainly for average pooled DNNs. Maybe add one more sentence to say it is possible to use *deactivated* GAP features too
%\\

%This is advantageous since it is straightforward to find the mean and standard deviation of a linear combination of Gamma distributed random variables. 
Suppose we have $N$ deactivated GAP features, each represented by random variables $G_i, i = 1,2,...,N$, with their respective mean and variances denoted as $\mu_{G,i}, \sigma^2_{G,i}$. In the case where an average pooled DNN is considered, the equations for $\mu_{G,i}$ and $\sigma^2_{G,i}$ are Eq. \ref{eq:gapsum_mean} and Eq. \ref{eq:gapsum_var} respectively. In the case where the deactivation layer is used, the equations for  $\mu_{G,i}$ and $\sigma^2_{G,i}$ are Eq. \ref{eq:deact_mu} and Eq. \ref{eq:deact_sigma} respectively.

%, where $X_i$ follows a Gamma distribution with shape parameter $a_i$, scale parameter $s_i$ and location parameter $l_i$. It can be shown that the mean and variance of these Gamma distributions are $\mu_i = a_is_i + l_i/s_i$ and $\sigma^2_i = a_is_i^2$ respectively. 
Then, suppose the fully connected classification layer has the following weights on these $N$ deactivated GAP features: $\{\alpha_i\}_{i=1}^N$. Then, let $O$ denote the random variable of the output layer before sigmoid activation, where:
%\[
$O = \sum^N_{i=1} \alpha_iG_i$.
%\]

Then, by the linearity of the expectation operator, the mean of $O$ is:
\begin{equation}
\mu_O = \sum^N_{i=1} \alpha_i\mu_{G,i}
\label{eq:out_mu}
\end{equation}

Similarly, it can be shown that the variance is:
\begin{equation}
\sigma^2_O = \sum^N_{i=1} \alpha^2_i \sigma_{G,i}^2 + 2\sum_{1\leq i < j \leq N} \alpha_i\alpha_jCov_D(i,j)
\label{eq:out_sigma}
\end{equation}
where $Cov_D(i,j)$ is the covariance of the $i^{th}$ and $j^{th}$ deactivated GAP features given in Eq. \ref{eq:deact_cov}.
Thus, by the central limit theorem, the distribution of $O$ can be approximated by the normal distribution:
\[
f(x) = \frac{1}{\sqrt{2\sigma_O}}\exp\left(
- \frac{(x - \mu_O)^2}{2\sigma_O^2}
\right)
\]

\subsection{KL-Divergence of Positive and Negative Class Output Values}
Using the normal distribution approximation detailed in the previous section, we can now directly find the KL divergence of the pre-sigmoid outputs of a DNN between positive and negative classes for both the average pool DNN and non-linearly activated DNN.
% we may want to connect all the things from the last convolutional layer to here now
% TODO - maybe want to say a bit more about mu and sigma for positive and negative data using eq out mu and out sigma?
In general, suppose we are given two normal distributions, say $p_-(x)$ and $p_+(x)$, with mean and standard deviation from Eq. \ref{eq:out_mu} and \ref{eq:out_sigma}, $(\mu_-,\sigma_-)$ and $(\mu_+,\sigma_+)$ respectively, their KL divergence has a particularly simple form:
\begin{equation}
    K( p_+, p_- ) = \log( \sigma_- ) - \log( \sigma_+ ) + \frac{\sigma_+^2 + (\mu_+ - \mu_-)^2}{2\sigma_-} - \frac{1}{2}
\label{eq:kl_div_func}
\end{equation}

\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{CVPR_eyepacs.pdf}
\caption{ROC curves for three CNNs on Eyepacs dataset: Average pooling CNN, proposed Activation CNN and Google CNN}
\label{fig:roc_eyepacs}
\end{figure}

\section{Application:KL Divergence Optimisation}
In this section, we describe a method for directly optimising the KL divergence with respect to the tunable parameters in the aggregation block and the fully connected classification layer. This is achieved using gradient ascent and has many similarities with the stochastic gradient descent approach commonly used. The main difference is that we directly optimise the distribution in order to maximise KL divergence instead of individual batches of examples.

% TODO - Q: what is the advantage of optimising at a distribution level instead of individual batches of subsets of training examples?

Our task is now to find the gradients of the KL-divergence function (Eq. \ref{eq:kl_div_func}. Our proposed mathematical formulation in Section \ref{sec:agg_blocks} established a nested sequence of functions that link various learnable parameters and the KL-divergence function.
Thus, the chain rule can be used to efficiently derive the required derivatives in a similar manner to backpropagation.
% TODO - describe the different parameters that can be tuned and how to obtain the total derivative for each of the weights/parameters.

\subsection{Gradients for KL-divergence Optimisation}
We start by obtaining the partial derivatives of $K$ with respect to its input parameters:
\begin{eqnarray*}
\frac{\partial K}{\partial \sigma_+} & = & -\frac{1}{\sigma_+} + \frac{\sigma_+}{\sigma_-^2} \\
\frac{\partial K}{\partial \sigma_-} & = & \frac{1}{\sigma_-} - \frac{\sigma_+^2 + (\mu_+ - \mu_-)^2}{\sigma_-^3} \\
\frac{\partial K}{\partial \mu_+} & = & \frac{\mu_+ - \mu_-}{\sigma_-^2} \\
\frac{\partial K}{\partial \mu_-} & = & \frac{\mu_- - \mu_+}{\sigma_-^2}
\end{eqnarray*}
We will now proceed to determine the derivatives for the parameters in the different layers considered in Section \ref{sec:agg_blocks}.

\subsubsection{Fully Connected Classification Layer Gradients}
Suppose we want to obtain the gradient of the weight $\alpha_i, i \in \{1,...,N\}$ in the FC classification layer. This is done by obtaining the total derivative $dK/d\alpha_i$:
\[
\frac{dK}{d\alpha_i} = \frac{\partial K}{\partial \sigma_-}\frac{d\sigma_-}{d\alpha_i} + \frac{\partial K}{\partial \sigma_+}\frac{d\sigma_+}{d\alpha_i} + \frac{\partial K}{\partial K}\frac{d\mu_-}{d\alpha_i} + \frac{\partial K}{\partial \mu_+}\frac{d\mu_+}{d\alpha_i}
\]
where the output distribution
The derivatives of the output distributions with respect to the weights are:
\begin{eqnarray*}
\frac{d\mu_-}{d\alpha_i} & = & \mu^-_{G,i} \\
\frac{d\mu_+}{d\alpha_i} & = & \mu^+_{G,i} \\
\frac{d\sigma_-}{d\alpha_i} & = & \frac{1}{\sigma_-}\left(\alpha_i(\sigma^-_{G,i})^2 + \sum^N_{j=1,j\neq i}\alpha_jCov^-(i,j)\right) \\
\frac{d\sigma_-}{d\alpha_i} & = & \frac{1}{\sigma_+}\left(\alpha_i(\sigma^+_{G,i})^2 + \sum^N_{j=1,j\neq i}\alpha_jCov^-(i,j)
\right)
\end{eqnarray*}
% TODO - need to explain that Cov has +ve and -ve, and also \mu_{G,i} has positive and negative, \sigma_{G,i} too

Compiling all the above total derivatives for all $i = 1,2,...,N$ gives is the gradient vector for adjusting the fully connected classification layer weights:
\[
\delta(\mathbf{\alpha}) = \left(\frac{dK}{d\alpha_i}\right)_{i=1}^N
\]

\subsubsection{Deactivation Layer Gradients}
We recall that the deactivation layer parameter is $\gamma$ and is present in Equations \ref{eq:deact_mu} and \ref{eq:deact_sigma}.
The total derivative of $K$ with respect to the deactivation parameter is:
\begin{equation}
\frac{dK}{d\gamma}  =  \sum_{*\in\{+,-\}}\left[\frac{\partial K}{\partial\mu_*}\left(\sum^N_{i=1}\alpha_i\frac{d\mu^*_{G,i}}{d\gamma}\right) + \frac{\partial K}{\partial \sigma_*}\frac{d\sigma_*}{d\gamma}
\right]
\end{equation}
Here we denote the mean of the $i^{th}$ GAP variable ($\mu_{G,i}$ of Eq. \ref{eq:gapsum_mean}) obtained using only positively labelled images with the superscript $+$ as $\mu^+_{G,i}$. Similarly, the standard deviation for only positive images is denoted as $\sigma^+_{G,i}$. In the event of raising the standard deviation to some power $k$, we denote it as $(\sigma^+_{G,i})^k$.
The same applies for negative labelled images but with the superscript of $-$ instead.

In the derivatives of the GAP variables with respect to the deactivation parameter $\gamma$ given below, we use $*\in \{+,-\}$ as a placeholder for the positive and negative subscripts. We start with differentiating Eq. \ref{eq:deact_mu} (with the appropriate subscripts to denote which GAP feature, and superscript to denote the label):
\begin{eqnarray*}
\frac{d\mu^*_{G,i}}{d\gamma} & = & \frac{1}{\Gamma(a_i)}\left[
\gamma ({s^*_i})^{\gamma - 1}\Gamma(\gamma + a^*_i) + \right.\\
&& \left. (s^*_i)^\gamma \Gamma( \gamma + a^*_i ) \psi(\gamma + a^*_i)
\right]
\end{eqnarray*}
where $a^*_i,s^*_i$ are the shape and scale parameters of the $i^{th}$ GAP feature for label $*$, with distribution with the form of Eq. \ref{eq:gap_pdf} and $\psi(\gamma + a_i)$ denotes the digamma function, a special function defined as the logarithmic derivative of the Gamma function.

Next, the derivative of the output layer variance is obtained by differentiating Eq. \ref{eq:out_sigma} with respect to $\gamma$:
\begin{eqnarray*}
\frac{d\sigma_*}{d\gamma} & = & \sum^N_{i=1}\alpha^2_i 2\sigma_{G,i}\frac{d\sigma^*_{G,i}}{d\gamma}
\end{eqnarray*}
with the $i^{th}$ GAP feature deactivated variance derivative given as:
\begin{eqnarray*}
\frac{d\sigma^*_{G,i}}{d\gamma} & = & \frac{({s^*_i})^{2\gamma}}{\Gamma(a^*_i)}\left[ \frac{1}{s_i^*}\left( \Gamma(a_i^* + 2\gamma) - \frac{\Gamma(a_i^* + \gamma)^2}{\Gamma(a_i^*)}\right) +  \right. \\
&& \left. 
\Gamma(a_i^* + 2\gamma)\psi(a_i^* + 2\gamma) - \frac{\Gamma(a_i^* + \gamma)^2\psi(a_i^* + \gamma)}{\Gamma(a_i^*)}
\right]
\end{eqnarray*}

We now provide the partial derivatives that will be backpropagated to the non-linear activation layer (if used).

\subsubsection{Exponential Activation Layer Gradients}
There are two parameters that can be adjusted in the exponential activation layer, the scaling factor $\alpha$ (not to be confused with the FC classification layer weights $\alpha_i$) and the exponential factor $\beta$.

\subsubsection{Powered Activation Layer Gradients}

\section{Experimental Results and Analysis}
\label{sec:exp}
In this section, we validate the intuitions and proposed approach on three diverse computer vision tasks:image category classification, medical image detection, instance image retrieval. Each tasks poses unique challenges. For each tasks we briefly describe the datasets, the network architectures and key experiment parameters. 

\subsection*{Image category classification of Flowers dataset}
This section presents the performance of our Activation CNN on image classification task. The Activation CNN consists of baseline ResNet50 network. The last convolutional layer output of ResNet50 is passed to activation layer which amplifies the feature map values in a non-linear fashion: dampening the weaker responses and improving the discriminative power of stronger responses. The activation layer is followed by Global Average Pooling (GAP) layer, de-activation layer and fully-connected (FC) layer. We use the Flowers dataset, containing 3700 images belonging to five classes, to train and validate proposed method. We convert the multi-class classification problem into 1-vs-all problems to support the theoretical results build up in Section \ref{sec:agg_blocks} and Section \ref{sec:class_kl}.

\begin{table}[h]
\caption{Classification accuracy of Average pool CNN and Activation CNN}
\label{tab:flower-table}
\begin{tabular}{|l|c|c|}
\hline
\multicolumn{1}{|c|}{} & Average pool CNN & Activation CNN \\ \hline 
Daisy & 95.2 \% & 96.7 \% \\ \hline
Dandelion & 94.6 \% & 96.1 \% \\ \hline
Rose & 91.8 \% & 91.2 \% \\ \hline
Sunflower & 94.2 \% & 95.4 \% \\ \hline
Tulip & 91.5 \% & 91.8 \% \\ \hline
\end{tabular}
\end{table}

Table \ref{tab:flower-table} compares the performance of Activation CNN with Average pooling CNN (ResNet50 + GAP +FC layers). It can be seen that the Activation CNN has better classification accuracy on majority of classes, compared to Average pool CNN.

\subsection*{Detection of Diabetic Retinopathy in Retinal Fundus Photographs}
In this section, we develop and validate our proposed algorithm for automated detection of diabetic retinopathy (DR) in retinal fundus photographs of EyePACS dataset (88702  images). The overall architecture consists of a baseline InceptionV4 network, activation layer, GAP layer, deactivation layer, FC layer and classification layer. The CNN is trained on 80\% of Eyepacs dataset using cross-entropy loss and validated on remaining 20\% images using classification accuracy. 

Figure \ref{fig:roc_eyepacs} shows the Receiver Operating Characteristic (ROC) curve of three CNNs: proposed activation CNN, average pooling CNN and state-of-the art Google CNN. It can be observed that activation CNN performs better than average pooling CNN and comparably to Google CNN. It is important to that Google used significantly larger number of images for training (128175 images), used human graders to remove poor-quality images and performed ensembling of 10 CNNs, compared to our approach. 

\subsection*{Instance level retrieval of landmarks}
We develop and validate our proposed algorithm for image retrieval task. A baseline ResNet101 model is used, with activation pooling, trained with Arcface loss on Google landmarks retrieval v2 dataset. We evaluate the trained CNN on independent landmark retrieval datasets, Revisited Oxford ($R$Oxf) and Revisited Paris ($R$Par), using medium and hard setups referred as $R$Oxf$M$, $R$Par$M$, $R$Oxf$H$ and $R$Par$H$. 

It can be observed from Table \ref{MobileNettab} the our Activation CNN performs significantly better that the state-of-the-art on all four benchmarks.

\begin{table}[htbp]
\caption{Retrieval accuracy for three CNNs on retrieval datasets}
\label{MobileNettab}
\resizebox{\columnwidth}{!}{\begin{tabular}{|l|c|c|c|c|}
\hline & $R$Oxf$M$ & $R$Oxf$H$ & $R$Par$M$ & $R$Par$H$ \\ \hline \hline
Average pooling CNN &75.9  &55.2  &87.1 &73.9\\ \hline
ResNet101+ArcFace \cite{weyand2020google} &76.2 &55.6 & 87.3 &74.2 \\ \hline
Activation CNN &\bf{77.4}  &\bf{58.5} &\bf{88.3} &\bf{76.5}  \\ \hline

\end{tabular}}
\end{table}

% Question - do we want a section showing the distributions at the different activation layer ?
\subsection{Prediction of DNN KL-Divergence}
In this section, we show that our method is able to predict the KL-divergence of DNNs across a range of different problems. We consider the cases where only average pooling and when non-linear activation was used. The results can be seen in Fig. \ref{fig:kl_plot}. Here, we see the scatter plots showing the predicted KL divergence using our proposed framework against the KL divergence obtained directly from the values of the output node (positive class) of the DNN. 
Each point corresponds to a particular type of activation used (blue circles for exponential activation, black cross average pooling) and class chosen as the positive label. We see that in general, the points lie close to the diagonal line, showing that our predicted KL divergences are not too different to their corresponding observed KL divergences.

We can also see the DNN output node distributions for the CIFAR10 and Flowers data in Fig. \ref{fig:cifar_flowers_out_distrib} and EyePACs data in Fig. \ref{fig:eyepacs_out_distrib}. In these figures, we plot the predicted output normal distributions (solid curve) with the histogram built using the output node values. Black is used to denote negative class labels and red denotes positive classes. It can be seen that our prediction agrees well with the underlying histogram in the case of CIFAR10. This is also the case for the EyePACs dataset. In the case of the Flowers dataset, due to a small number of images, our histograms are sparse, but we can still see that our predicted distributions agree in general with the underlying histograms. 
% Do we want to say why the mean is a bit offset in some cases?

\begin{figure*}
    \centering
    \begin{tabular}{ccccccccccc}
    AvPl&\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls0.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls1.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls2.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls3.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls4.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls5.pdf}
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls6.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls7.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls8.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_out_cls9.pdf} \\
    ExpPl&\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls0.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls1.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls2.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls3.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls4.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls5.pdf}
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls6.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls7.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls8.pdf} 
    &\includegraphics[align=c, width=0.08\linewidth]{cifar_imgs/cifar_exp_out_cls9.pdf} \\
    &C1 & C2 & C3 & C4 & C5 & C6 & C7 & C8 & C9 &C10
    \end{tabular}\\
    CIFAR10 Dataset\\
    \begin{tabular}{cccccc}
    AvPl&\includegraphics[align=c, width=0.15\linewidth]{flower_imgs/flower_daisy_avp.pdf} &
          \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_dan_avp.pdf}  
         & \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_rose_avp.pdf} & 
         \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flowers_sunflower.pdf} & 
         \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_tulip_avp.pdf} \\
         ExpPl &\includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_daisy_exp.pdf} 
         & \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_dan_exp.pdf}  
         & \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_rose_exp.pdf} & 
         \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_sunflower_exp.pdf} & 
         \includegraphics[align=c,width=0.15\linewidth]{flower_imgs/flower_tulip_exp.pdf} \\
          &Daisy & Dandl. & Rose & SunFlw. & Tulip
    \end{tabular} \\
    Flowers Dataset
    
    \caption{Examples of predicted output node distributions (red and black curves) and observed underlying histograms. Black represents images with negative labels, whilst red represents images with positive labels.}
    \label{fig:cifar_flowers_out_distrib}
\end{figure*}
% Eyepacs dataset results
\begin{figure}
    \centering
    \begin{tabular}{ccc}
    %Average Pool & Exp. Pool & KL-Div.\\
    \includegraphics[width=0.4\linewidth]{imgs/eyepacs_avpool.pdf} & \includegraphics[width=0.4\linewidth]{imgs/eyepacs_exppool.pdf} \\
    AvPl & ExpPl
    \end{tabular} 
    \caption{EyePACs Dataset predicted output node distributions (red and black curves) and observed underlying histograms. Black represents images with negative labels, whilst red represents images with positive labels.}
    \label{fig:eyepacs_out_distrib}
\end{figure}
\begin{figure}
    \centering
    \begin{tabular}{ccc}
         \includegraphics[width=0.33\linewidth]{imgs/cifar_kl.pdf}&  
         \includegraphics[width=0.33\linewidth]{imgs/flowers_kl.pdf} & 
         \includegraphics[width=0.33\linewidth]{imgs/eyepacs_kl.pdf} \\
         CIFAR10 & Flowers & EyePACs
    \end{tabular}
    \caption{Scatter plots of predicted (x-axis) against observed (y-axis) KL-divergence of the DNN output node.The green diagonal line on the right plot indicates when the predicted and observed KL divergence are equal. Blue circles indicate exponential activation, and black crosses indicate average pooling.}
    \label{fig:kl_plot}
\end{figure}

\section{Conclusions}
\label{sec:conclusions}
In this paper, we have proposed a novel mathematical formulation that allowed for the analytical modelling of probability distributions of output values of layers involved with deep feature aggregation. We considered both the common average pooling DNN and non-linearly activated aggregation methods. We have found that when the last convolutional layer outputs are modelled using Gamma distributions, it is possible to derive the distributions of the various layers involved in the aggregation process. From this, the weigths of the fully connected classification layer can be used to give an normal distribution approximation to the output node distribution, allowing the KL divergence between classes. We have shown experimentally that our KL divergence predictions are accurate across three different datasets and tasks.
%\section{Open Questions}
% 1) It is unknown in what situations the Gamma distribution will be too bad a fit for the outputs of the last convolutional layers
% 2) The covariance between the filters are very important in determining the variance in the output node distribution
% 3) 

==> new_conclusion.tex <==
In this paper, we have proposed a novel mathematical formulation that allowed for the analytical modelling of probability distributions of layer activations involved with nonlinear deep feature aggregation. 
In this paper, we have carried out a theoretical study of the distributions of activations in the aggregation process of a deep net. To achieve this, we proposed a novel mathematical formulation that allowed for the analytical modelling of probability distributions of layer activations involved with nonlinear deep feature aggregation.  
Using a mixed discrete-continuous distribution for modelling the output values of convolutional layers, we derived the output distributions for each layer in the aggregation block.
We then showed how these distributions can be used to model the output value distributions of a classification DNN. This immediately allowed us to obtain the KL divergence of the DNN. Importantly, we now have a direct link between the learnable parameters for layers starting from the aggregation block and the DNN KL divergence. From this, we made a theoretical observation of how the covariance of pre-aggregation deep features can influence the KL divergence and thus, classification performance of a deep net. In particular, we have found that an increase in covariance of convolutional layer activations leads to a decreased KL divergence, confirming existing intuition on the need for decorrelated deep features for good DNN accuracy. The model predictions were then verified on classification tasks from two different datasets and DNN models, where our models were shown to have good agreement with the experimental results.

%We have found that when the last convolutional layer outputs are modelled using a mixed distribution consisting of a discrete point distribution and continuous Gamma distributions, it is possible to derive the distributions of the various layers involved in the aggregation process. From this, the weights of the fully connected classification layer can be used to give an normal distribution approximation to the output node distribution, allowing the KL divergence between classes. We have shown experimentally that our KL divergence predictions are accurate across different datasets and tasks. We have also found that the covariance between different deep features play a significant role in determining the variances of output responses of a DNN. We can see that a greater covariance between the outputs of the last convolutional layer reduces the KL divergence of a DNN. 


==> new_intro.tex <==
In recent years, deep neural networks (DNN) have shown excellent performance across a wide range of tasks, for example, image classification and retrieval.
One element that is almost ubiquitous in state-of-the-art DNN architectures is the use of aggregation processes, where deep features are combined together into a more compact representation, with the intuition that stronger (i.e. higher valued) features represent important information. 
The aggregation process can occur from the local level to global levels. One of the earliest use of aggregation was by Fukushima \cite{Fukushima1980}, where average pooling was introduced to reduce the size of convolutional images. Later, Weng et al. \cite{maxpool_weng} introduced the max-pooling layer in the Cresceptron framework, whereby activation values of a patch is replaced by its maximum value. The aggregation process was then extended by Lin et al. \cite{lin2014network} to act on a more global level, where the all the convolutional activations of a filter were replaced by a single aggregated average value. This brought the advantage of improved robustness to overfitting and spatial translations of the input. Greater emphasis can be placed on strong features in the aggregation process by using more generalised activation pooling methods \cite{GEM,HusainPAMI}, where the global average pooling layer was sandwiched between two non-linear transformations. This was found to have significantly improved the accuracy of the DNN when applied on image retrieval tasks. 

%
It can be argued that the pooling process, is as important as the feature extracting convolutional filters in a deep net. This applies especially to the global pooling since it determines the separability of features that ultimately defines the accuracy of a DNN. As an example, it was found in \cite{HusainPAMI} that the retrieval or classification performance of DNNs correlates strongly with an increase in the KL divergence of its outputs.
% Question - what is the reason for the above statement? 
%
In order to better understand the usefulness of aggregation, we need to understand the quality of the aggregated features. One way of achieving this is by using information theoretic methods such as KL divergence. In order to do this, we need knowledge about the distributions of activations throughout the aggregation process. To our knowledge, this paper presents a first attempt in the theoretical study of the distributions of aggregated features. We will also show that these models agree well with results from DNN models used in practice.
% Knowledge about how the distribution of convolutional features change as it passes through the aggregation process can be very useful. 
%One aspect of the aggregation process that remains less studied is the understanding of how the distribution of convolutional features change as it passes through the aggregation process. The value of understanding the output distributions of layers in a deep net is exemplified by the Batch Normalisation method, which allowed very deep nets to be trained. This was achieved by stabilising the output value distributions of intermediate layers inside a DNN. Our work is therefore concerned about developing a mathematical framework for analysing the distributions of deep features at each point of the aggregation process.

%The use global aggregation methods has the advantage of making the DNN agnostic to the input image resolution. 
% One point - knowledge about how information flows through a DNN allows us to predict its uncertainty. 
%It was found in \cite{HusainPAMI} that the retrieval or classification performance of DNNs correlates strongly with an increase in the KL divergence of its outputs. Therefore, knowledge of how the KL divergence is theoretically related to earlier layers of a DNN will provide valuable knowledge into further improving the performance of existing DNNs. This in turn requires knowledge of the statistical distribution of different layers in DNNs.

==> summary.tex <==
\section{Summary of contents}
Contents will include:
\begin{itemize}
    \item Exponential Non-linear activation for improved classification
    \item Theoretical Analysis of KL divergence of DNNs
    \item - theoretical model of the whole non-linear aggregated block (exp-GAP-deact).
    \item - - Gamma distributed convolutional output values
    \item - - Derivation of exponentiated convolutional activation distribution
    \item - - Distribution of deactivated GAP feature values
    \item - Explicit formulation of KL divergence for standard DNNs and non-linearly activated DNNs.
    \item - Analysis of difference between KL divergences of standard DNNs and those with an activation block added.
    \item - Experimental Results to support the above. CIFAR, Caltech 101, Eyepacs
\end{itemize}
